State-of-The-Art Sparse Direct Solvers

In this chapter we will give an insight into modern sparse elimination methods. These are driven by a preprocessing phase based on combinatorial algorithms which improve diagonal dominance, reduce fill-in, and improve concurrency to allow for parallel treatment. Moreover, these methods detect dense submatrices which can be handled by dense matrix kernels based on multithreaded level-3 BLAS. We will demonstrate for problems arising from circuit simulation, how the improvements in recent years have advanced direct solution methods significantly.

==> Regression/preamble.tex <==
\usepackage{etex}
\usepackage{cite}
\ifCLASSINFOpdf
\usepackage{graphicx}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi


\usepackage{multicol,multirow}
\usepackage{amsmath,amsfonts, amssymb, mathtools}
%\usepackage{subfig}
\usepackage{enumitem}
%\usepackage{color}
\usepackage{empheq}
\usepackage[dvipsnames]{xcolor}
\usepackage[normalem]{ulem}  
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.8}
% \pgfplotsset{compat=newest}
\usetikzlibrary{patterns}

\usepackage{pgfplotstable, booktabs}  % booktabs for \toprule etc
%\usepgfplotslibrary{external} 
%\tikzexternalize



\usepackage{csvsimple}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks,pdfhighlight=/O,pdfdisplaydoctitle=true,urlcolor=blue,pdfpagemode=UseOutlines,pdfstartview=FitV, pdfpagetransition=Glitter,citecolor=blue, colorlinks=true, pagebackref=false, pdfpagelabels=true,linkcolor=blue, linktocpage=true]{hyperref}

\usepackage{algpseudocode}
\usepackage{algorithm}

%\footnotesize\bgroup\par\centering\@IEEEtabletopskipstrut{\normalfont\footnotesize {#1.}\nobreakspace\scshape #2}\par\addvspace{0.5\baselineskip}\egroup%
%\makeatletter
%\newcommand\fs@norules{\def\@fs@cfont{\scshape\footnotesize}\let\@fs@capt\floatc@plain
%  \def\@fs@pre{\hrule height.8pt depth0pt \kern5pt}%
%  \def\@fs@post{\kern5pt\hrule height.8pt depth0pt \kern5pt}
%  \def\@fs@mid{\kern5pt\hrule\kern5pt}
%  \let\@fs@iftopcapt\iftrue}
%\makeatother
%\floatstyle{norules}
%\restylefloat{algorithm}


%\definecolor{excelblue}{RGB}{101,170,233}
%\definecolor{excelred}{RGB}{221,132,125}
%\definecolor{excelgreen}{RGB}{215,239,143}
%\definecolor{excelpurple}{RGB}{194,178,232}
%\definecolor{excelcyan}{RGB}{178,237,255}
%\definecolor{excelpurple}{RGB}{235,125,60}
%\definecolor{excelblue}{RGB}{76,104,167} 
%\definecolor{excelred}{RGB}{152,75,68}
%\definecolor{excelgreen}{RGB}{125,136,69}
%\definecolor{excelcyan}{RGB}{79,122,142}

%\definecolor{mycolor1}{RGB}{130,220,202}
%\definecolor{mycolor2}{RGB}{79,122,142}  %{92,78,49}   
%\definecolor{mycolor3}{RGB}{170,35,3} 
%\definecolor{mycolor4}{RGB}{207,170,114}
%\definecolor{mycolor4}{RGB}{79,122,142}  %{92,78,49}   
%\definecolor{mycolor5}{RGB}{80,135,63}
%\definecolor{mycolor6}{RGB}{255,140,190}


% Spectral colormap
\definecolor{mycolor1}{HTML}{D7191C}
\definecolor{mycolor2}{HTML}{FDAE61}
\definecolor{mycolor3}{HTML}{FFFFBF}
\definecolor{mycolor4}{HTML}{ABDDA4}
\definecolor{mycolor5}{HTML}{2B83BA}

% PuOr colormap with black MIDDLE
%\definecolor{mycolor1}{HTML}{E66101}
%\definecolor{mycolor2}{HTML}{FDB863}
%\definecolor{mycolor3}{HTML}{000030}
%\definecolor{mycolor4}{HTML}{B2ABD2}
%\definecolor{mycolor5}{HTML}{5E3C99}

% RdBu
%\definecolor{mycolor1}{HTML}{CA0020}
%\definecolor{mycolor2}{HTML}{F4A582}
%\definecolor{mycolor3}{HTML}{F7F7F7}
%\definecolor{mycolor4}{HTML}{92C5DE}
%\definecolor{mycolor5}{HTML}{0571B0}

% BrBg
%\definecolor{mycolor1}{HTML}{A6611A}
%\definecolor{mycolor2}{HTML}{DFC27D}
%\definecolor{mycolor3}{HTML}{F7F7F7}
%\definecolor{mycolor4}{HTML}{80CDC1}
%\definecolor{mycolor5}{HTML}{018571}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}

%\newcommand{\RefereeA}[1]{\textcolor{mycolor1}{#1}}
%\newcommand{\RefereeB}[1]{\textcolor{mycolor2}{#1}}
%\newcommand{\RefereeC}[1]{\textcolor{mycolor3}{#1}}
%\newcommand{\RefereeD}[1]{\textcolor{mycolor4}{#1}}
%\newcommand{\RefereeE}[1]{\textcolor{mycolor5}{#1}}
%\newcommand{\RefereeF}[1]{\textcolor{mycolor6}{#1}}

\newcommand{\RefereeA}[1]{\textcolor{black}{#1}}
\newcommand{\RefereeB}[1]{\textcolor{black}{#1}}
\newcommand{\RefereeC}[1]{\textcolor{black}{#1}}
\newcommand{\RefereeD}[1]{\textcolor{black}{#1}}
\newcommand{\RefereeE}[1]{\textcolor{black}{#1}}
\newcommand{\RefereeF}[1]{\textcolor{black}{#1}}


%\newcommand{\revisionDel}[1]{\Midline{#1}}
%\newcommand{\revisionDel}[1]{\ifmmode\text{\sout{\ensuremath{#1}}}\else\sout{#1}\fi}
\newcommand{\revisionDel}[1]{}

\newcommand{\pmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\pvec}[1]{\begin{pmatrix}#1\end{pmatrix}}


\graphicspath{{./pic/}}
\DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\newcommand{\eref}[1]{(\ref{#1})}
\newcommand{\sref}[1]{section \ref{#1}}
\newcommand{\fref}[1]{Fig. \ref{#1}}
\newcommand{\tref}[1]{Table \ref{#1}}
%\newcommand{\algref}[1]{Alg. \ref{alg:#1}}

\newcommand{\Cal}[1]{\mathcal{#1}}
\newcommand{\Poly}[1]{\mathrm{#1}}
\newcommand{\PolyPartition}[1]{\mathcal{#1}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\Set}[1]{\mathbb{#1}}
\newcommand{\PP}{\Poly{P}}
\newcommand{\PaP}{\PolyPartition{P}}
\newcommand{\PaJ}{\PolyPartition{J}}
\newcommand{\R}[1]{\Set{R}^{#1}}
\newcommand{\ComplexSet}[1]{\Set{C}^{#1}}
\newcommand{\One}{\Set{I}}
\newcommand{\N}[1]{\Set{N}^{#1}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}

\renewcommand{\l}{\left}
\renewcommand{\r}{\right}
\newcommand{\st}{\mbox{subject to}}




%%%%%%%%%%%%%%%%%%%%%%%
%%% Added by Drosos %%%
%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage[svgnames]{xcolor}
\usepackage[framemethod=tikz]{mdframed}
\usepackage[customcolors]{hf-tikz}
\usetikzlibrary{shadows}

\newmdenv[
%settings={\refstepcounter{exa}},
leftmargin=0pt,
rightmargin=0pt,
linewidth=1pt,
innerleftmargin=-1pt,
innerrightmargin=3pt,
innertopmargin=0.25\baselineskip,
roundcorner=6pt,
backgroundcolor=gray!10,
linecolor=black,
frametitle=,%(MPOPF),%~\theexa,
frametitlefont=\scshape\color{red!70!black},
shadow=true
]{mdexample}

\def\a{{\mathbf a}}
\def\v{{\mathbf v}}
\def\x{{\discr{x}}}
\def\w{{\discr{w}}}
\def\b{{\discr{b}}}
\def\u{{\discr{u}}}
\def\r{{\discr{r}}}
\def\z{{\discr{z}}}
\def\s{{\discr{s}}}
\def\c{{\discr{c}}}
\def\y{{\discr{y}}}
\def\e{{\discr{e}}}
\def\l{{\discr{l}}}

\def\g{{\mathbf g}}
\def\p{{\mathbf p}}
\def\q{{\mathbf q}}
\def\h{{\mathbf h}}

\newcommand{\ve}[1]{{\mathbf v}^{#1}}
\newcommand{\pe}[1]{{\mathbf p}^{#1}}
\newcommand{\pes}[2]{{\mathbf p}^{#1}_{#2}}
%\newcommand{\mabs}[1]{\text{abs}\left({#1}\right)}
\newcommand{\mabs}[1]{\left|{#1}\right|}
\newcommand{\mdiag}[1]{\text{diag}\left({#1}\right)}
\newcommand{\mexp}[1]{\text{exp}\left({#1}\right)}
\newcommand{\cplxe}[2]{\underline{#1}^{#2}}
\newcommand{\Complex}[1]{\underline{#1}}
\def\vcn{\Complex{\v}_n}
\def\vn{{\v}^{n}}
\def\pn{{\p}^{n}}
\def\pnmax{{\p}^{\text{max}}}
\def\pnmin{{\p}^{\text{min}}}
\def\pgmax{{\p}^{\text{G,max}}}
\def\pgmin{{\p}^{\text{G,min}}}
\def\qgmax{{\q}^{\text{G,max}}}
\def\qgmin{{\q}^{\text{G,min}}}
\def\psmax{{\p}^{\text{S,max}}}
\def\psmin{{\p}^{\text{S,min}}}
\def\qsmax{{\q}^{\text{S,max}}}
\def\qsmin{{\q}^{\text{S,min}}}
\def\qnmax{{\q}^{\text{max}}}
\def\qnmin{{\q}^{\text{min}}}
\def\pgn{{\p}^{\text{G},n}}
\def\qgn{{\q}^{\text{G},n}}
\def\pg{{\p}^{\text{G}}}
\def\qg{{\q}^{\text{G}}}
\def\ps{{\p}^{\text{S}}}
\def\qs{{\q}^{\text{S}}}
\newcommand{\psci}{{\p}^{\text{Sc},i}}
\newcommand{\psdi}{{\p}^{\text{Sd},i}}
\newcommand{\pscn}{{\p}^{\text{Sc}}_n}
\newcommand{\psdn}{{\p}^{\text{Sd}}_n}
\newcommand{\psd}{{\p}^{\text{Sd}}}
\newcommand{\pscni}[2]{{\p}^{\text{Sc},{#1}}_{#2}}
\newcommand{\psdni}[2]{{\p}^{\text{Sd},{#1}}_{#2}}
\newcommand{\qscni}[2]{{\q}^{\text{Sc},{#1}}_{#2}}
\newcommand{\qsdni}[2]{{\q}^{\text{Sd},{#1}}_{#2}}
\newcommand{\psni}[1]{{\p}^{\text{S},#1}}
\newcommand{\pni}[1]{{\p}_{#1}}
\def\qn{{\q}^{n}}
% \def\Yl{\cplxe{\mathbf{Y}}{\text{l}}}
% \def\Yb{\cplxe{\mathbf{Y}}{\text{b}}}
\def\Yl{\Complex{\mathbf{Y}}^{\text{L}}}
\def\Yb{\cplxe{\mathbf{Y}}{\text{B}}}
\def\ibi{\cplxe{\mathbf i}{\text{B},i}}
\def\ib{\Complex{\mathbf i}^{\text{B}}}
\def\il{\Complex{\mathbf i}^{\text{L}}}
\def\ili{\cplxe{\mathbf i}{\text{L},i}}
\def\scomplex{\Complex{\mathbf s}}
\def\sL{\Complex{\mathbf s}^{\text{L}}}
\def\sLi{\Complex{\mathbf s}^{\text{L},i}}
\def\sB{\Complex{\mathbf s}^{\text{B}}}
\def\sBi{\Complex{\mathbf s}^{\text{B},i}}
\def\slnmax{ {\mathbf s}^{\text{L,max}} }
\def\sdn{\cplxe{\mathbf s}{\text{D}}_n}
\def\sd{\Complex{\mathbf s}^{\text{D}}}
\def\pd{{\p}^{\text{D}}}
\def\pdk{{\p}^{\text{D},k}}
\def\qd{{\q}^{\text{D}}}
\def\sdi{\Complex{\mathbf s}^{\text{D},i}}
\def\sg{\Complex{\mathbf s}^{\text{G}}}
\def\sS{\Complex{\mathbf s}^{\text{S}}}
\def\Asone{{\mathbf A}^{\p,1}}
\def\Astwo{{\mathbf A}^{\p,2}}
\def\As{{\mathbf A}^{\text{S}}}
\def\Es{{\mathbf E}^{\text{S}}}
\def\Ezero{{\mathbf E}^{\text{0}}}
\def\apmax{{\mathbf a}^{\p, \text{max}}}
\def\apmin{{\mathbf a}^{\p, \text{min}}}

\def\bTheta{{\boldsymbol \Theta}}
\def\btheta{{\boldsymbol \theta}}
\def\bthetan{{\boldsymbol \theta}^n}
\def\bxi{{\boldsymbol \xi}}
\def\blambda{{\boldsymbol \lambda}}
\def\bepsilon{{\boldsymbol \epsilon}}
\def\bepsilonmax{{\boldsymbol \epsilon}^\text{max}}
\def\bepsilonmin{{\boldsymbol \epsilon}^\text{min}}
\def\bepsilonmaxS{{\boldsymbol \epsilon}^\text{max}_\text{S}}
\def\bepsilonminS{{\boldsymbol \epsilon}^\text{min}_\text{S}}
\def\bepsilonmaxSi{{\boldsymbol \epsilon}^\text{max}_{\text{S},i}}
\def\bepsilonminSi{{\boldsymbol \epsilon}^\text{min}_{\text{S},i}}
\def\bepsilonmaxSk{{\boldsymbol \epsilon}^\text{max}_{\text{S},k}}
% \def\bepsilon{{\boldsymbol E}}
% \def\bepsilonmax{{\boldsymbol E}^\text{max}}
% \def\bepsilonmin{{\boldsymbol E}^\text{min}}
\def\bLambda{{\boldsymbol \Lambda}}
\def\bmu{{\boldsymbol \mu}}




\def\O{{\discr{O}}}
\def\Sc{{\discr{S}}}
\def\G{{\discr{G}}}
\def\P{{\discr{P}}}
\def\A{{\discr{A}}}
\def\B{{\discr{B}}}
\def\Ib{{\discr{I}}}
% \def\Bs{{\discr{B}^\text{S}}}
\def\Bs{{\mathbf{B}^\text{S}}}
\def\E{{\mathbf {E}}}
\def\C{{\discr{C}}}
\def\D{{\discr{D}}}
\def\V{{\discr{V}}}
\def\U{{\discr{U}}}
\def\W{{\discr{W}}}
\def\Z{{\discr{Z}}}
\def\L{{\discr{L}}}

\def\Xmin{{X^\text{min}}}
\def\Xmax{{X^\text{max}}}
\def\Smin{{S^\text{min}}}
\def\Smax{{S^\text{max}}}

\def\DXmin{{\tilde{X}^\text{min}}}
\def\DXmax{{\tilde{X}^\text{max}}}
\def\DSmin{{\tilde{S}^\text{min}}}
\def\DSmax{{\tilde{S}^\text{max}}}

\def\DXmink{{\tilde{X}^\text{min}_k}}
\def\DXmaxk{{\tilde{X}^\text{max}_k}}
\def\DSmink{{\tilde{S}^\text{min}_k}}
\def\DSmaxk{{\tilde{S}^\text{max}_k}}
\def\DXminkinv{({\tilde{X}^\text{min}_k)^{-1}}}
\def\DXmaxkinv{({\tilde{X}^\text{max}_k)^{-1}}}
\def\DSminkinv{({\tilde{S}^\text{min}_k)^{-1}}}
\def\DSmaxkinv{({\tilde{S}^\text{max}_k)^{-1}}}



\def\0{{\mathbf 0}}

\def\nbi{{n_b}}
\def\nfi{{n_f}}
\def\ngi{{n_g}}
\def\nxi{{n_x}}
\def\nzi{{n_z}}

\def\Nf{{N_f}}
% \def\Nb{{N_b}}
% \def\Ng{{N_g}}
% \def\Ns{{N_s}}
% \def\Nl{{N_\text{l}}}
% \def\Ngzero{{N_g^{0}}}
\def\Nb{{N_\text{B}}}
\def\Ng{{N_\text{G}}}
\def\Ns{{N_\text{S}}}
\def\Nl{{N_\text{L}}}
\def\Nd{{N_\text{D}}}
\def\Ngzero{{N_\text{G0}}}
\def\Nx{{N_x}}
\def\Nz{{N_z}}
% \def\Cbl{\mathbf{C}^{\text{bl}}}
% \def\Cblone{\mathbf{C}^{\text{bl,1}}}
% \def\Cbltwo{\mathbf{C}^{\text{bl,2}}}
\def\Cb{\mathbf{C}^{\text{B}}}
\def\Cbl{\mathbf{C}^{\text{L}}}
\def\Cblone{\mathbf{C}^{\text{L,1}}}
\def\Cbltwo{\mathbf{C}^{\text{L,2}}}
% \def\Cgb{\mathbf{C}^{\text{gb}}}
\def\Cgb{\mathbf{C}^{\text{G}}}
\def\Csb{\mathbf{C}^{\text{S}}}
\def\Csbzero{\mathbf{C}^{\text{S}0}}
\def\asmax{\mathbf{a}^{\text{S,max}}}
\def\asmin{\mathbf{a}^{\text{S,min}}}

\def\esmax{{\bepsilon}^{\text{S,max}}}
\def\esmin{{\bepsilon}^{\text{S,min}}}
\def \KKT{{\mathbf{\tilde{\Hess}}}}

\newcommand{\Hess}{\discr{H}}
\newcommand \discr[1]{{\boldsymbol{#1}}}   % how does it work with def and arguments ???
\newcommand{\Jac}{\discr{J}}
\newcommand{\vNull}{\discr{0}}

\newcommand{\HYPEROPT}{{\small BELTISTOS}}
\newcommand{\MATPOWER}{{\small MATPOWER}}
\newcommand{\PARDISO}{{\small PARDISO}}
\newcommand{\IPOPTPARDISO}{{\small IPOPT}}
\newcommand{\MIPS}{{\small MIPS}}
\newcommand{\KNITRO}{{\small KNITRO}}
\newcommand{\IPOPT}{{\small IPOPT}}
\newcommand{\KKTn}{{N_H}}

\newcommand{\iu}{\boldsymbol{\imath}}
\makeatletter
\newcommand*{\transpose}{%
	  {\mathpalette\@transpose{}}%
}
\newcommand*{\@transpose}[2]{%
	    % #1: math style
	      % #2: unused
	        \raisebox{\depth}{$\m@th#1\intercal$}%
}
\makeatother



\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\diag}{diag}

\def\minim{\mathop{\hbox{\rm minimize}}}
\def\subject{\text{\rm subject to}}
% \def\subject{\text{\rm s.t.}}
\def\minimize#1{{\displaystyle\minim_{#1}}}
    
\def\problemIP#1#2#3#4#5#6{\fbox
   {\begin{tabular*}{0.47\textwidth}
    {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
      #1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
         & $\subject$      & $#4$ & $ $ \\[5pt]
         & & $#5$ & $ $ \\[5pt]
         & & $#6$ & $ $ \\
    \end{tabular*}}}
    



==> figures/RJGraphs/barPlot_all.tex <==
\begin{tikzpicture}
\pgfplotstableread{\rjDataFileName}\datatable
\begin{axis}[name=symb,
width=0.39\textwidth, height=4cm, 
ybar,
bar width=3.5pt, 
ymode=normal, 
log origin=infty,
ymin=0,
%ymax=12,
axis lines*=left, 
ymajorgrids, yminorgrids,
%xticklabels from table={\datatable}{THREADS},
xticklabels={1,2,4,8,16},
xtick={1, 2, 3, 4, 5, 6, 7, 8},
xticklabel style={align=center, rotate=0, xshift=-0.0cm, anchor=north, font=\scriptsize},
%ytick={0,2,...,12},
try min ticks=7,
enlarge y limits={value=0.17,upper},
%yticklabels={$10^{-1}$, , , , , , , , $10^0$, , , , , , , , ,$10^1$},
yticklabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
%xlabel style={font=\scriptsize},
%ylabel=\ifrjYLabel {Performance Improvement} \else {} \fi,
%xlabel={Benchmark},
%legend style={at={(1.0,1.07)},fill=white,legend cell align=left,align=right,draw=white!85!black,font=\scriptsize,legend columns=4}
legend style={at={(1.0,1.25)},fill=white,legend cell align=left,align=right,draw=white!85!black,font=\tiny,legend columns=4},
title=\rjTitle,
every axis title/.style={below right,at={(0,1)},font=\footnotesize,yshift=5pt,xshift=1pt,fill=white}
]
\ifrjYLabel
   \pgfplotsset{ylabel={Performance Improvement}}
\else
\fi
\ifrjXTicks
   \pgfplotsset{xlabel=threads,xlabel style={font=\footnotesize,yshift=4pt}}
\else
   \pgfplotsset{xmajorticks=false}
\fi
%\addplot[fill=mycolor0] table[x=ID, y=TTOTAL] {\datatable};
%\addlegendentry{Overall time}
\addplot[fill=mycolor1, postaction={pattern=north east lines}] table[x=ID, y=MKL_PARDISO] {\datatable}; 
\ifrjLegend
\addlegendentry{MKL PARDISO}
\fi
%\addplot[fill=mycolor2, postaction={pattern=north west lines}] table[x=ID, y=TFEVAL] {\datatable}; 
%\addlegendentry{Function evaluations}
\addplot[fill=mycolor3, postaction={pattern=crosshatch}] table[x=ID, y=PARDISO_6_0] {\datatable}; 
\ifrjLegend
\addlegendentry{PARDISO 6.2}
\fi
\end{axis}
\end{tikzpicture}

